Towards Sharp Analysis for Distributed Learning with Random Features

In recent studies, the generalization properties for distributed learning and random features assumed the existence of the target concept over the hypothesis space. However, this strict condition is not applicable to the more common non-attainable case. In this paper, using refined proof techniques, we first extend the optimal rates for distributed learning with random features to the non-attainable case. Then, we reduce the number of required random features via data-dependent generating strategy, and improve the allowed number of partitions with additional unlabeled data. Theoretical analysis shows these techniques remarkably reduce computational cost while preserving the optimal generalization accuracy under standard assumptions. Finally, we conduct several experiments on both simulated and real-world datasets, and the empirical results validate our theoretical findings.

==> 6-biography.tex <==

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\vspace{-2cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/biography-lijian.pdf}}]
  {\bf Jian Li} received the Ph.D. degree in Institute of Information  Engineering, Chinese Academy of Sciences, Beijing, China, in 2020.\\
  He is currently a researcher at the Institute of Information  Engineering, Chinese Academy of Sciences.
  %at Inception Institute of Artificial Intelligence (IIAI), Abu Dhabi, UAE.
  %He spent two years as a postdoctoral fellow at King Abdullah University of Science and Technology (KAUST), Saudi Arabia.
  His research interests include  statistical machine learning, large-scale kernel methods, and semi-supervised learning.
  \vspace{-2cm}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/biography-liuyong.pdf}}]
  {\bf Yong Liu} received the Ph.D. degree in computer science from Tianjin University, Tianjin, China, in 2016.\\
  He is currently an associate researcher at Gaoling School of Artificial Intelligence, Renmin University of China.
  \vspace{-2cm}
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/biography-wangweiping.pdf}}]
{\bf Weiping Wang} received the Ph.D. degree in computer science from Harbin Institute of Technology, China, in 2008.\\
He is currently a professor at Institute of Information Engineering, Chinese Academy of Sciences,
National Engineering Research Center for Information Security,
and the National Engineering Laboratory for Information Security Technology.
% His research interests include database and storage systems.
% %He has more than 30 publications in major journals and international conferences.
\end{IEEEbiography}

